Geometric Packing under Non-uniform Constraints

We study the problem of discrete geometric packing. Here, given weighted regions (say in the plane) and points (with capacities), one has to pick a maximum weight subset of the regions such that no point is covered more than its capacity. We provide a general framework and an algorithm for approximating the optimal solution for packing in hypergraphs arising out of such geometric settings. Using this framework we get a flotilla of results on this problem (and also on its dual, where one wants to pick a maximum weight subset of the points when the regions have capacities). For example, for the case of fat triangles of similar size, we show an O(1)-approximation and prove that no \PTAS is possible.

==> figs/prefix.tex <==
% All style files are available from
% http://wwww.uiuc.edu/~sariel/research/latex/
\usepackage[breaklinks]{hyperref} % comment out if you do not have it
\usepackage{graphicx}
\usepackage[active]{srcltx} % comment out if you do not have it
%\usepackage{fullpage}%
%\usepackage{wide}%
\usepackage{euscript}%
\usepackage{xspace}%
\usepackage{color}%
\usepackage{amsmath}%
\usepackage{paralist}%
\usepackage{theorem}%
\usepackage{picins}%
\usepackage{boxedminipage}
\usepackage{enumerate}
\usepackage{picins}
\usepackage{multirow}

%wider ``normal'' margins
% Margins - stuff like that
\setlength{\textwidth}{6.5in}
\setlength{\topmargin}{0.0in}
\setlength{\headheight}{0in}
\setlength{\headsep}{0.0in}
\setlength{\textheight}{9in}
\setlength{\oddsidemargin}{0in}
\setlength{\evensidemargin}{0in}

\newcommand{\xparagraph}[1]{{\smallskip\textsf{#1}}}


\newcommand{\Opt}{\mathrm{opt}}%
\newcommand{\OptLP}{\mathrm{opt}_{\text{LP}}}
\newcommand{\PTAS}{\Term{P{T}AS}\xspace}

\newcommand{\ts}{\hspace{0.6pt}}%
\renewcommand{\th}{\si{th}\xspace}

\newcommand{\scl}{\Delta}%
\newcommand{\sclC}{\alpha}

\newcommand{\Circle}{C}

% \si{something} - emacs spell checker ignores something
\providecommand{\si}[1]{#1}

\newcommand{\AlinaThanks}[1]{%
   \thanks{Department of Computer Science; %
      University of Illinois; %
      201 N. Goodwin Avenue; %
      Urbana, IL, 61801, USA; %
      {\tt \si{ene}1\atgen{}\si{uiuc}.\si{edu}}; {\tt
         \si{\url{http://www.cs.uiuc.edu/\string~ene1/}}.} #1}}



\newcommand{\BenThanks}[1]{\thanks{Department of Computer Science;
      University of Illinois; %
      201 N. Goodwin Avenue; %
      Urbana, IL, 61801, USA; %
      {\tt \si{raichel}2\atgen{}\si{uiuc}.\si{edu}}; %
      {\tt \url{\si{http://www.cs.uiuc.edu/\string~\si{raichel2}}}}%
      . %
      #1}}

\newcommand{\atgen}{\symbol{'100}}
\newcommand{\SarielThanks}[1]{\thanks{Department of Computer Science;
      University of Illinois; 201 N. Goodwin Avenue; Urbana, IL,
      61801, USA; {\tt \si{sariel}\atgen{}\si{uiuc.edu}}; %
      {\tt \url{http://www.uiuc.edu/\string~sariel/}.} #1}}

\newcommand{\emphind}[1]{\emph{#1}\index{#1}}
\definecolor{blue25}{rgb}{0,0,0.55}%
\newcommand{\emphic}[2]{%
   \textcolor{blue25}{%
      \textbf{\emph{#1}}}%
   \index{#2}}

\newcommand{\emphi}[1]{\emphic{#1}{#1}}
\newcommand{\pth}[2][\!]{#1\left({#2}\right)}
\newcommand{\rpth}[2][]{#1\left({#2}\right)}

% problem names
\definecolor{red25}{rgb}{0.4,0,0.0}%

\newcommand{\PStyle}[1]{\textcolor{red25}{\textsc{#1}}}
\newcommand{\PackRegions}       {\PStyle{{Pack{}Regions}}\xspace}
\newcommand{\PackPoints}        {\PStyle{{Pack{}Points}}\xspace}
\newcommand{\PackHGraph}        {\PStyle{{HGraph{}Packing}}\xspace}%
\newcommand{\PackHalfspaces}    {\PStyle{{Pack{}Halfspaces}}\xspace}
%\newcommand{\PackPlanesInRays}{\textsc{Pack{}Planes{}In{}Rays}\xspace}
\newcommand{\PackRaysInPlanes}  {\PStyle{{Pack{}Rays{}In{}Planes{}}}\xspace}
\newcommand{\PackPointsInDisks} {\PStyle{{Pack{}Points{}In{}Disks}}\xspace}
\newcommand{\PackRectsInPnts}   {\PStyle{{Pack{}Re{}ct{}s{}In{}Points}}\xspace}
\newcommand{\PackBoxesInPnts}   {\PStyle{{Pack{}Boxes{}In{}Points}}\xspace}
\newcommand{\PackPntsInSkyline} {\PStyle{{Pack{}Pnts{}In{}Skyline}}\xspace}
\newcommand{\PackPntsInRects}   {\PStyle{Pack{}Pnts{}In{}Rect{}s}\xspace}

%\newcommand{\script#1}{\mathcal{#1}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}%
\newtheorem{definition}[theorem]{Definition}
\newtheorem{defn}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{problem}[theorem]{Problem}%

{\theorembodyfont{\rm} \newtheorem{remark}[theorem]{Remark}}

\newcommand{\brc}[1]{\left\{ {#1} \right\}}


\newcommand{\ObjSet}{\EuScript{D}}%
\newcommand{\ObjSetA}{X}%


\newcommand{\Disk}{\mathsf{d}}%
\newcommand{\DiskSet}{\EuScript{D}}

\newcommand{\PlaneSet}{\EuScript{H}}%
\newcommand{\plane}{\mathsf{h}}%

\newcommand{\HalfspaceSet}{\EuScript{S}}%
\newcommand{\Halfspace}{\mathsf{h}}%
\newcommand{\RaySet}{\EuScript{R}}%
\newcommand{\Ray}{\mathsf{r}}%

\newcommand{\RectSet}{\EuScript{B}}
\newcommand{\RectSetA}{\EuScript{D}}

\newcommand{\BoxSet}{\EuScript{B}}
\newcommand{\rect}{\mathsf{b}}


\newcommand{\VSetA}{X}%
\newcommand{\VSetB}{Y}%
\newcommand{\VSetC}{Z}%
\newcommand{\VSetD}{U}%
\newcommand{\VOpt}{V_{\Opt}}%

\newcommand{\Inst}{{I}}

\newcommand{\Term}[1]{\textsf{#1}}%

\newcommand{\VC}{\Term{VC}\xspace}
\newcommand{\LP}{\Term{LP}\xspace}%
\newcommand{\HyperLP}{\textsc{Hypergraph-LP}\xspace}
\newcommand{\APX}{\Term{AP{X}}\xspace}%
\newcommand{\APXHard}{\Term{AP{X}-hard}\xspace}%
\newcommand{\MAXSNP}{\Term{MAX S{}NP}\xspace}%
\newcommand{\NPHard}{\Term{NP-Hard}\xspace}%
\newcommand{\NPH}{\Term{NPH}\xspace}%
\renewcommand{\P}{\Term{P}\xspace}%
\newcommand{\NP}{\Term{NP}\xspace}%
\newcommand{\obj}{b}%
\newcommand{\hedge}{f}%


\newcommand{\conflict}{h}%
\newcommand{\conflictSet}{\mathcal{H}}%
\newcommand{\RSample}{\mathsf{R}}%

\newcommand{\graph}{{G}}%
\newcommand{\hgraph}{\mathsf{G}}%
\newcommand{\VSet}{\mathsf{V}}%
\newcommand{\HESet}{\mathsf{E}}%

\newcommand{\vertex}{v}%
\newcommand{\weight}[1]{w\pth{#1}}%

%\newcommand{\RSet}{\mathcal{R}}%
%\newcommand{\RSet}{\mathcal{S}}%
\newcommand{\RSet}{\mathcal{C}}%
\newcommand{\OSet}{\mathcal{O}}

%\newcommand{\pnt}{{\mathsf{p}}}
\newcommand{\Energy}{\EuScript{E}}

\newcommand{\EnergyX}[2][\!]{\EuScript{E}\pth[#1]{#2}}

\newcommand{\XSays}[2]{{
      {$\rule[-0.12cm]{0.2in}{0.5cm}$\fbox{\tt
            #1:} }
      #2
      \marginpar{#1}
      {$\rule[0.1cm]{0.3in}{0.1cm}$\fbox{\tt
            end}$\rule[0.1cm]{0.3in}{0.1cm}$}
      }
   }
\newcommand{\sariel}[1]{{\XSays{Sariel}{#1}}}
\newcommand{\Sariel}[1]{{\XSays{Sariel}{#1}}}


\newcommand{\cRelax}{\phi}
\newcommand{\forceX}[2][\!]{\rho\pth[#1]{#2}}
\newcommand{\forceY}[2]{\rho_{#1}\pth{#2}}%
\newcommand{\resistC}{\eta}%
\newcommand{\resistX}[1]{\resistC\pth{#1}}%
\newcommand{\resistY}[2]{\resistC\pth{#1, #2}}
\newcommand{\resistZ}[3]{\resistC_{#1}\pth{#2, #3}}
\newcommand{\constA}{c_1}%
\newcommand{\indep}{\Term{I{N}D{E}P}\xspace}%
\newcommand{\Union}[2][\!]{\mathsf{U}\pth[#1]{#2}}
\newcommand{\union}[2][\!]{\mathsf{u}\pth[#1]{#2}}
\renewcommand{\Re}{{\rm I\!\hspace{-0.025em} R}}

\newcommand{\mc}{\nu}

\newcommand{\aftermathA}{\par\vspace{-\baselineskip}}%

\newcommand{\mba}     {\rule[0.0cm]{0.0cm}{0.36cm}} % really small
\newcommand{\mbb}     {\rule[0.0cm]{0.0cm}{0.38cm}} % really small
\newcommand{\mbc}     {\rule[0.0cm]{0.0cm}{0.40cm}} % really small
\newcommand{\mbd}     {\rule[0.0cm]{0.0cm}{0.42cm}} % really small
\newcommand{\mbe}     {\rule[0.0cm]{0.0cm}{0.44cm}} % really small
\newcommand{\mbf}     {\rule[0.0cm]{0.0cm}{0.46cm}} % really small
\newcommand{\mbg}     {\rule[0.0cm]{0.0cm}{0.48cm}} % really small
\newcommand{\mbh}     {\rule[0.0cm]{0.0cm}{0.50cm}} % really small
\newcommand{\mbi}     {\rule[0.0cm]{0.0cm}{0.52cm}} % really small
\newcommand{\mbj}     {\rule[0.0cm]{0.0cm}{0.54cm}} % really small
\newcommand{\MakeBig} {\rule[-.2cm]{0cm}{0.4cm}}
\newcommand{\MakeSBig}{\rule[0.0cm]{0.0cm}{0.38cm}} % really small

\newcommand{\seclab}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}

\newcommand{\problab}[1]{\label{prob:#1}}
\newcommand{\probref}[1]{Problem~\ref{prob:#1}}

\newcommand{\thmlab}[1]{{\label{theo:#1}}}%
\newcommand{\thmref}[1]{Theorem~\ref{theo:#1}}%

\providecommand{\deflab}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}


\newcommand{\corlab}[1]{\label{cor:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}

\newcommand{\itemlab}[1]{\label{item:#1}}
\newcommand{\itemref}[1]{(\ref{item:#1})}

\newcommand{\lemlab}[1]{\label{lemma:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lemma:#1}}

\newcommand{\figlab}[1]{\label{figure:#1}}
\newcommand{\figref}[1]{Figure~\ref{figure:#1}}

\newcommand{\TwoFigures}[6]{\begin{tabular}{cc}
       \begin{minipage}{0.48\linewidth}
           \begin{center}
               \centerline{\includegraphics[#1]{{#2}}}
           \end{center}
       \end{minipage}
       &
       \begin{minipage}{0.48\linewidth}
           \centerline{\includegraphics[#4]{{#5}}}
       \end{minipage}
%       \\
       ~\\[-0.2cm]
       {#3} & {#6}
   \end{tabular}}


\newenvironment{proof}{\trivlist\item[]\emph{Proof}:}%
{\unskip\nobreak\hskip 1em plus 1fil\nobreak%
   \myqedsymbol%$\Box$
   \parfillskip=0pt%
   \endtrivlist}
\newenvironment{proofof}[1]{\smallskip\noindent{\bf Proof of #1:}}%
{\unskip\nobreak\hskip 1em plus 1fil\nobreak%
   \myqedsymbol%$\Box$
   \parfillskip=0pt%
   \endtrivlist}

\newcommand{\myqedsymbol}{\rule{2mm}{2mm}}
\newcommand{\cardin}[1]{\left| {#1} \right|}
\newcommand{\pbrcx}[1]{\left[ {#1} \right]}
\newcommand{\Ex}[2][\!]{\mathop{\mathbf{E}}#1\pbrcx{#2}}
\newcommand{\Prob}[1]{\mathop{\mathbf{Pr}}\!\pbrcx{#1}}
\newcommand{\sep}[1]{\,\left|\, {#1} \MakeBig\right.}
\newcommand{\permut}[1]{\left\langle {#1} \right\rangle}%

\newcommand{\capacityX}[1]{\#(#1)}

\newcommand{\Pnum}{\psi}%
\newcommand{\eqlab}[1]{\label{equation:#1}}
\newcommand{\Eqref}[1]{\si{Eq}.~(\ref{equation:#1})}
\providecommand{\ds}{\displaystyle}


\newcommand{\local}{\mathsf{L}}%
\newcommand{\indepSet}{\mathsf{I}}%
\newcommand{\eps}{\varepsilon}%

\newcommand{\seg}{\mathsf{s}}%
\newcommand{\SegSet}{\mathsf{S}}%
\newcommand{\fleq}[2]{f_{\leq{#1}} \pth{#2}}%
\newcommand{\feq}[2]{F_{{#1}} \pth{#2}}%

\newcommand{\Family}{\mathcal{F}}
\newcommand{\InducedX}[2]{#1_{#2}}
\newcommand{\Alg}{\ensuremath{\mathtt{alg}}\xspace}
\newcommand{\iright}{i_{\mathrm{right}}}
\newcommand{\ileft}{i_{\mathrm{left}}}
\newcommand{\remove}[1]{}

\newcommand{\ceil}[1]{\left\lceil {#1} \right\rceil}
\newcommand{\floor}[1]{\left\lfloor {#1} \right\rfloor}
\newcommand{\Turan}{T{u}r\'an\xspace}

\newcommand{\etal}{\textit{et~al.}\xspace}

% Nicer footnotes symbols

\usepackage{pifont}%

\usepackage[symbol*]{footmisc}

\DefineFNsymbols*{stars}[text]{%
   {\ding{172}} %
   {\ding{173}} %
   {\ding{174}} %
   {\ding{175}} %
   {\ding{176}} %
   {\ding{177}} %
   {\ding{178}} %
   {\ding{179}} %
   {\ding{180}} %
   }
\setfnsymbol{stars}

%%BeginIpePreamble
%% ^^^^^^^^^^^^^^ Do not delete!

\newcommand{\DLeftX}[1]{#1_{\leftarrow}}
\newcommand{\DLeftTopX}[1]{#1_{\nwarrow}}
\newcommand{\DLeftBottomX}[1]{#1_{\swarrow}}
\newcommand{\DRightX}[1]{#1_{\rightarrow}}
\newcommand{\Tri}{\triangle}%
\newcommand{\TriL}{\DLeftX{\Tri}}%
\newcommand{\TriLT}{\DLeftTopX{\Tri}}%
\newcommand{\TriLB}{\DLeftBottomX{\Tri}}%
\newcommand{\TriR}{\DRightX{\Tri}}%

\newcommand{\TriSet}{\EuScript{T}}%
\newcommand{\TriSetLB}{\DLeftBottomX{\TriSet}}%
\newcommand{\TriSetLT}{\DLeftTopX{\TriSet}}
\newcommand{\TriSetR} {\DRightX{\TriSet}}


\newcommand{\pnt}{{\mathsf{p}}}%
\newcommand{\pntA}{{\mathsf{q}}}%
\newcommand{\pntB}{{\mathsf{s}}}

\newcommand{\Line}{\ell}
\newcommand{\LineA}{\wp}

\newcommand{\PntSet}{\mathsf{P}}%
\newcommand{\PntSetA}{Q}%

%%EndIpePreamble
%% ^^^^^^^^^^^^^^ Do not delete!

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "packing"
%%% End: 


==> generate_submission <==
#! /bin/tcsh -f 

rm -f junk/err_submission

pdflatex "\def\confMode{TRUE}\input{"packing.tex"}"  > /dev/null
bibtex packing > /dev/null
pdflatex "\def\confMode{TRUE}\input{"packing.tex"}" > /dev/null
pdflatex "\def\confMode{TRUE}\input{"packing.tex"}" > /dev/null
pdflatex "\def\confMode{TRUE}\input{"packing.tex"}" >>  junk/err_submission

mkdir conf >& /dev/null
cp packing.pdf conf/packing_conf.pdf


pdflatex packing.tex  > /dev/null
bibtex packing > /dev/null
pdflatex packing.tex > /dev/null
pdflatex packing.tex > /dev/null
pdflatex packing.tex >>  junk/err_submission

cp packing.pdf conf/packing_full.pdf

cd conf

pdftk packing_conf.pdf packing_full.pdf cat output packing_submit.pdf
cp packing_submit.pdf ..



